A Theory of Universal Learning

How quickly can a given class of concepts be learned from examples? It is common to measure the performance of a supervised machine learning algorithm by plotting its "learning curve", that is, the decay of the error rate as a function of the number of training examples. However, the classical theoretical framework for understanding learnability, the PAC model of Vapnik-Chervonenkis and Valiant, does not explain the behavior of learning curves: the distribution-free PAC model of learning can only bound the upper envelope of the learning curves over all possible data distributions. This does not match the practice of machine learning, where the data source is typically fixed in any given scenario, while the learner may choose the number of training examples on the basis of factors such as computational resources and desired accuracy. In this paper, we study an alternative learning model that better captures such practical aspects of machine learning, but still gives rise to a complete theory of the learnable in the spirit of the PAC model. More precisely, we consider the problem of universal learning, which aims to understand the performance of learning algorithms on every data distribution, but without requiring uniformity over the distribution. The main result of this paper is a remarkable trichotomy: there are only three possible rates of universal learning. More precisely, we show that the learning curves of any given concept class decay either at an exponential, linear, or arbitrarily slow rates. Moreover, each of these cases is completely characterized by appropriate combinatorial parameters, and we exhibit optimal learning algorithms that achieve the best possible rate in each case. For concreteness, we consider in this paper only the realizable case, though analogous results are expected to extend to more general learning scenarios.

==> macros.tex <==
%\newlength{\dhatheight}
%\newcommand{\doublehat}[1]{%
%    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
%    \addtolength{\dhatheight}{-0.35ex}%
%    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
%    \smash{\hat{#1}}}}

\newlength{\dhatheight}
\newcommand{\hhatDS}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
\newcommand{\hhatTS}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}    
\newcommand{\hhatS}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\scriptstyle{\hat{#1}}}}%
    \addtolength{\dhatheight}{-0.175ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
\newcommand{\hhatSS}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\scriptscriptstyle{\hat{#1}}}}%
    \addtolength{\dhatheight}{-0.07ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
\newcommand{\hhat}[1]{\mathchoice{\hhatDS{#1}}{\hhatTS{#1}}{\hhatS{#1}}{\hhatSS{#1}}}

\newcommand{\region}{\mathcal{U}}
\newcommand{\Px}{\mathcal{P}}
\newcommand{\PXY}{\mathcal{P}_{XY}}
\newcommand{\PXYR}[1]{\mathcal{P}_{#1}}
%\newcommand{\PXYR}{\mathcal{P}_{\region}}
\newcommand{\Risk}{{\rm R}_{\loss}}
\newcommand{\Rademacher}{\hat{\phi}}
\newcommand{\loss}{\ell} % loss function
\newcommand{\maxloss}{\bar{\loss}} % largest possible loss value
\newcommand{\transform}{\psi_{\loss}} % the psi-transform
\newcommand{\tsyba}{\alpha} % Tsybakov exponent for 0-1 loss
\newcommand{\tsybca}{a} % Tsybakov leading constant for 0-1 loss
\newcommand{\tsybb}{\beta} % Tsybakov exponent for surrogate loss
\newcommand{\tsybcb}{b} % Tsybakov leading constant for surrogate loss
\newcommand{\TN}{{\rm MT}} % set of distributions satisfying Tsybakov noise
\newcommand{\BN}{{\rm BN}} % set of distributions satisfying Bounded noise
\newcommand{\RE}{{\rm RE}} % set of distributions satisfying the Realizable case
\newcommand{\AG}{{\rm AG}} % set of distributions satisfying a noise bound in the agnostic case
\newcommand{\BE}{{\rm BE}} % set of distributions satisfying a noise bound in the benign noise case 
\newcommand{\DL}{{\rm BC}} % set of distributions satisfying the diameter localization condition (Bernstein Class Assumption)
\newcommand{\RR}{{\rm RR}} % set of distributions from the work of Raginsky and Rakhlin, 2011
\newcommand{\s}{\mathfrak{s}}
\newcommand{\XTD}{{\rm XTD}} % extended teaching dimension
\newcommand{\TD}{{\rm TD}} % teaching dimension
\newcommand{\XPTD}{{\rm XPTD}} % extended partial teaching dimension
\newcommand{\entc}{q} % leading constant for entropy condition
\newcommand{\entrho}{\rho} % exponent for entropy condition
\newcommand{\g}{g} % a function
\newcommand{\h}{h} % a function (often a classifier)
\newcommand{\f}{f} % another function
\newcommand{\dc}{\theta} % the disagreement coefficient
\newcommand{\zc}{\varphi} % the sup of the ratio of the quantity from 
%\newcommand{\zc}{\sigma} % the sup of the ratio of the quantity from.  (old notation was \varphi, but I noticed Kamalika used \sigma in a talk)
\newcommand{\maxzc}{\hat{\zc}} % the maximum of \zc over the choice of \agtarget
\newcommand{\subcs}{\chi} % subregion compression set size
\newcommand{\ZC}{{\rm SubregionActive}} % subregion-based active learning algorithm
\newcommand{\supdc}{\hhat{\dc}} % the supremum (over distributions and targets) of the disagreement coefficient
\newcommand{\infsplit}{\hhat{\rho}} % infimum splitting index
\newcommand{\basicsplit}{\bar{\rho}} % the splitting index, without the Delta things, just that \C is (\rho,\eps,\tau)-splittable.
%\newcommand{\finitesplit}{\mathring{\rho}} % the limiting splitting index for a finitely discrete distribution
%\newcommand{\uniquesplit}{\sigma} % a variant of splitting where we specify one point responsible for each pair
\newcommand{\dd}{D} % doubling dimension (not sure what a good notation for this might be)
\newcommand{\capacity}{\tau} % the general capacity function
\newcommand{\mixcap}{\chi} % mixed capacity, where the numerator is prob of disagreement while denominator is loss diameter
\newcommand{\exreals}{\bar{\mathbb{R}}}
%\newcommand{\G}{\mathcal{G}}
\newcommand{\J}{{\rm J}} % entropy integral from van der Vaart & Wellner 2011
\newcommand{\D}{{\rm D}} % loss diameter ; might alternatively consider the notation \sigma for this?
\newcommand{\dist}{\Delta} % \Px(x : sign(g(x)) neq sign(h(x)))
\newcommand{\radius}{{\rm radius}} % max distance from target
\newcommand{\Transform}{\Gamma_{\loss}} %%% \Transform(er(h) - er(f*);P) \leq R(h;P) - R(f*;P)
\newcommand{\Epsilon}{\mathscr{E}}
\newcommand{\InvTransform}{\Epsilon_{\loss}}
\newcommand{\Functions}{\F^{*}} % set of all functions
\newcommand{\FunctionsXY}{\G^{*}} % set of functions mapping \X\times\Y \to [-\maxloss,\maxloss].
\newcommand{\Env}{{\rm F}} % envelope function
\newcommand{\bound}{\beta} % the noise bound for bounded noise
\newcommand{\BJM}{\Psi_{\loss}}
\newcommand{\zo}{{\scriptscriptstyle{01}}}
%\newcommand{\targtrunc}[2]{{#1}_{#2}^{\star}}
%\newcommand{\sgntrunc}[2]{{#1}_{#2}^{\pm}}
\newcommand{\spec}[1]{\mathring{#1}} % new special type of bound
\newcommand{\loose}[1]{\breve{#1}} % looser spec bound
\newcommand{\phiinv}[1]{\ddot{#1}} % just invert the phi term for sample size
\newcommand{\restinv}[1]{\dot{#1}} % inverse of the rest of the bound
\newcommand{\ERM}{{\rm ERM}}
\newcommand{\LC}{\Lambda} % label complexity in the pool-based (or stream-based) active learning model
\newcommand{\SC}{\mathcal{M}} % sample complexity of passive learning
\newcommand{\QC}{Q} % query complexity in the repeated query model
%\newcommand{\SC}{{\rm M}}
%\newcommand{\vc}{d}
\newcommand{\vc}{{\rm vc}}
\renewcommand{\dim}{d} % to be introduced as short-hand for VC dimension
\newcommand{\cs}{n} % sample compression size
\newcommand{\covering}{{\cal{N}}}
\newcommand{\G}{{\cal{G}}}
\newcommand{\conv}{{\rm conv}}
\newcommand{\Fbound}{\bar{B}} % bound on the functions
\newcommand{\metricbound}{\bar{d}_{\loss}} % bound on the pseudo-metric
\newcommand{\metric}{d_{\loss}} % pseudo-metric for the function values
\newcommand{\Lip}{L} % Lipschitz constant
\newcommand{\convc}{C_{\loss}} % constant factor in modulus of convexity lower bound
\newcommand{\convr}{r_{\loss}} % exponent in modulus of convexity lower bound
\newcommand{\modconv}{\bar{\delta}_{\loss}} % modulus of convexity
\newcommand{\Bracket}[1]{[#1]} % bracketing set given by upper and lower envelope functions
\newcommand{\Log}{{\rm Log}}
\newcommand{\polylog}{{\rm polylog}}
\newcommand{\Borel}{{\cal B}}
\newcommand{\BorelX}{{\cal B}_{\X}}

\newcommand{\Alg}{\mathcal{A}}
\newcommand{\CAL}{{\rm CAL}}
\newcommand{\ACAL}{RobustCAL}
\newcommand{\Shattering}{Shattering}
\newcommand{\RobustShattering}{RobustShattering}
\newcommand{\ZCPassive}{{\rm Algorithm~1}}
\newcommand{\conf}{\delta}
\newcommand{\eps}{\varepsilon}
\newcommand{\sfun}{\mathfrak{s}}
\newcommand{\X}{\mathcal X} % instance space
\renewcommand{\O}{O} % Big-O notation
\newcommand{\Y}{\mathcal Y} % label space
\newcommand{\alg}{\mathbb{A}} % learning algorithm
\renewcommand{\H}{\mathcal H} % hypothesis space
\renewcommand{\L}{\mathcal L} % labeled set
\newcommand{\U}{\mathcal U} % unlabeled set
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\target}{f^{\star}} % target function
\newcommand{\agtarget}{h^{\star}} % best classifier in the concept space
\newcommand{\cl}[1]{{\rm cl}(#1)} % closure
\newcommand{\er}{{\rm er}} % error rate
\newcommand{\core}{\partial} % disagreement core (or shatter core, when raised to a power)
\newcommand{\konst}{k} % the constant factor we lose in the sample complexity statement
\newcommand{\Ball}{{\rm B}}
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\newcommand{\ind}{\mathbbold{1}}
%\newcommand{\ind}{\mathbbm{1}}
\newcommand{\indpm}{\ind^{\pm}}
\newcommand{\hyp}{h} % hypothesis function
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\C}{\mathbb{C}} % concept space
\newcommand{\A}{\mathcal{A}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\sign}{{\rm sign}} % sign function
\newcommand{\T}{\mathcal T} % complete answer schemes
\renewcommand{\S}{\mathcal S} % generic collection of sets
\renewcommand{\P}{\mathbb P} % also probability
%\newcommand{\I}{\mathit I} % indicator function
%\newcommand{\R}{\mathit R} % overall risk functional
\newcommand{\nats}{\mathbb{N}} % natural numbers
\newcommand{\reals}{\mathbb{R}} % real numbers
\newcommand{\nts}{\mathbb{Z}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{{\rm Var}}
\newcommand{\Data}{\mathcal{Z}}
\newcommand{\DataX}{\mathbb{X}}
\newcommand{\DataY}{\mathbb{Y}}
%\newcommand{\dense}{\bar}
\newcommand{\dense}{} % this does nothing now
%\renewcommand{\alg}{DHM}
%\newcommand{\citet}{\cite}
%\newcommand{\citep}{\cite}
\newcommand{\diam}{{\rm diam}}
\newcommand{\DIS}{{\rm DIS}}
\newcommand{\DISXY}{\overline{\DIS}}
\newcommand{\DISF}{{\rm DISF}}
\newcommand{\DISFXY}{\overline{\DISF}}
\newcommand{\DISV}{D}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\argmin}{\mathop{\rm argmin}}
%\newcommand{\Tsybakov}{{\rm {Tsybakov}}}
%\newcommand{\vc}{d}
\newcommand{\Dset}{\mathbb{D}}
%\renewcommand{\limsup}{\mathop{\rm limsup}}
%\renewcommand{\liminf}{\mathop{\rm liminf}}
\newcommand{\hdc}{\tilde{\theta}} % higher-order disagreement coefficient
\newcommand{\bdim}{\tilde{d}} % shatter dimension
\newcommand{\dprob}{\tilde{\delta}_{f}}
\newcommand{\supp}{{\rm supp}} % the support of a probability measure
\newcommand{\RQCAL}{Algorithm 1} % the layered repeated queries modification of CAL
\newcommand{\Filter}{Subroutine 1} % the subroutine that repeatedly queries in a cell of the partition
\newcommand{\RealizableAlg}{Algorithm 0} % realizable-case algorithm based on repeated (1/2)-nets querying
\newcommand{\MembHalvingII}{{\sc Memb-Halving-2}} % hegedus memb-halving-2 algorithm
\newcommand{\truV}{V^{\star}} % version space consistent with all the target labels, even those not queried or noisy ones
\newcommand{\Split}{{\rm Split}} % for the splitting index definition
\renewcommand{\a}{a} % constant
\renewcommand{\b}{b} % constant
\renewcommand{\c}{c} % constant

\newcommand{\ignore}[1]{}
%\newcommand{\todo}[1]{}
\newcommand{\oldstuff}[1]{}

\newcommand{\new}[1]{{\color{red}{#1}}}
\newcommand{\shcomment}[1]{{\color{red}{#1}}}


%\newtheorem{theorem}{Theorem}[chapter]
%\newtheorem{definition}{Definition}[chapter]
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{definition}[theorem]{Definition}
%\theoremstyle{remark}
%\newtheorem{rem}{Remark}[section]
%\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{conjecture}[theorem]{Conjecture}

\newsavebox{\savepar}
\newenvironment{bigboxit}{\begin{center}\begin{lrbox}{\savepar}
%\begin{minipage}[h]{5.2in}
\begin{minipage}[h]{5.2in}
%\sffamily
\normalfont
\begin{flushleft}}
{\end{flushleft}\end{minipage}\end{lrbox}\fbox{\usebox{\savepar}}
\end{center}}

\newenvironment{bigbigboxit}{\begin{center}\begin{lrbox}{\savepar}
%\begin{minipage}[h]{5.2in}
\begin{minipage}[h]{5.8in}
%\sffamily
\normalfont
\begin{flushleft}}
{\end{flushleft}\end{minipage}\end{lrbox}\fbox{\usebox{\savepar}}
\end{center}}


\makeatletter
\newcommand{\vast}{\bBigg@{3}}
\newcommand{\Vast}{\bBigg@{4}}
\makeatother

